Advancing Real-time Pandemic Forecasting Using Large Language Models: A COVID-19 Case Study

Forecasting the short-term spread of an ongoing disease outbreak is a formidable challenge due to the complexity of contributing factors, some of which can be characterized through interlinked, multi-modality variables such as epidemiological time series data, viral biology, population demographics, and the intersection of public policy and human behavior. Existing forecasting model frameworks struggle with the multifaceted nature of relevant data and robust results translation, which hinders their performances and the provision of actionable insights for public health decision-makers. Our work introduces PandemicLLM, a novel framework with multi-modal Large Language Models (LLMs) that reformulates real-time forecasting of disease spread as a text reasoning problem, with the ability to incorporate real-time, complex, non-numerical information that previously unattainable in traditional forecasting models. This approach, through a unique AI-human cooperative prompt design and time series representation learning, encodes multi-modal data for LLMs. The model is applied to the COVID-19 pandemic, and trained to utilize textual public health policies, genomic surveillance, spatial, and epidemiological time series data, and is subsequently tested across all 50 states of the U.S. Empirically, PandemicLLM is shown to be a high-performing pandemic forecasting framework that effectively captures the impact of emerging variants and can provide timely and accurate predictions. The proposed PandemicLLM opens avenues for incorporating various pandemic-related data in heterogeneous formats and exhibits performance benefits over existing models. This study illuminates the potential of adapting LLMs and representation learning to enhance pandemic forecasting, illustrating how AI innovations can strengthen pandemic responses and crisis management in the future.

==> reference.tex <==
\section{References} 

Please use numerical references only for citations, and include the references within the manuscript file itself.  If you wish to use BibTeX, please copy the reference list from the .bbl file, paste it into the main manuscript .tex file, and delete the associated \bibliography and \bibliographystyle commands. Before submission, please ensure that the complete .tex file compiles successfully on your own system with no errors or warnings. There is no need to spend time visually formatting the manuscript: our style will be imposed automatically when the paper is prepared for publication.\\

\noindent Please do not cite web sites in the reference list — these should be listed separately, with the URLs in the Related Links section (see below).  If you are unsure if the website is a ‘Related link’ or should go in the ‘References’ section then identify if there is a publication date on the website.  If there is a publication date, it is likely that the item will be in the ‘References’ section.  If there is no publication date, it is likely that the item will be in the ‘Related Links’ section.\\

\noindent When citing a book, please indicate if you are citing a specific page range or chapter.  Otherwise, we presume that you are citing the entire book.  \\

\noindent \textbf{Highlighted references (optional)} Please select 5–-10 key references and provide a single sentence for each, highlighting the significance of the work.\\

\noindent\textbf{Acknowledgements}\\
E.g. Funding agencies.\\

\noindent\textbf{Author contributions}\\
Please describe the contributions made by each author.  Please use the initials of the individual author to explain these contributions.  These contributions are also required when you upload the files to our submission website.\\

\noindent\textbf{Competing interests}\\
Nature Journals require authors to declare any competing interests in relation to the work described. Information on this policy is available \href{http://www.nature.com/authors/policies/competing.html}{here}. \\



\noindent\textbf{Supplementary information (optional)}
If your article requires supplementary information, please include these files for peer-review. Please note that supplementary information will not be edited.

\begin{thebibliography}{10}

\bibitem{Hartkens_MICCAI_2002}
Hartkens, T., Hill, D.L., Castellano-Smith, A.D., Hawkes, D.J., Maurer, C.R., Martin, A.J., Hall, W.A., Liu, H. and Truwit, C.L.: Using points and surfaces to improve voxel-based non-rigid registration. In MICCAI, pp. 565-572. (2002)

\bibitem{zheng2020gman}
Zheng C, Fan X, Wang C, Qi J. Gman: A graph multi-attention network for traffic prediction. InProceedings of the AAAI Conference on Artificial Intelligence 2020 Apr 3 (Vol. 34, No. 01, pp. 1234-1241).

\bibitem{yao2019revisiting}
Yao H, Tang X, Wei H, Zheng G, Li Z. Revisiting spatial-temporal similarity: A deep learning framework for traffic prediction. InProceedings of the AAAI conference on artificial intelligence 2019 Jul 17 (Vol. 33, No. 01, pp. 5668-5675).

Zhao L, Song Y, Zhang C, Liu Y, Wang P, Lin T, Deng M, Li H. T-gcn: A temporal graph convolutional network for traffic prediction. IEEE Transactions on Intelligent Transportation Systems. 2019 Aug 22;21(9):3848-58.

\bibitem{xu2020spatial}
Xu M, Dai W, Liu C, Gao X, Lin W, Qi GJ, Xiong H. Spatial-temporal transformer networks for traffic flow forecasting. arXiv preprint arXiv:2001.02908. 2020 Jan 9.

\end{thebibliography}



==> tables/baseline.tex <==
\begin{table}[H]
\begin{center}
\caption*{Supplementary table 2: Selected hyperparameters for machine learning baselines}
 \label{tab:baseline}
\setlength{\tabcolsep}{8pt} % Default value: 6pt (column spacing)
\renewcommand{\arraystretch}{1.5} % Default value: 1 (row spacing)
\begin{tabular}{c|c|c|c|c}
\toprule[1.5pt]
\textbf{Model} & \textbf{Learning Rate} & \textbf{Sequence Length}  & \textbf{Hidden Layer Size} & \textbf{Number of Layers} \\ \hline
LSTM   & 0.00025        & 4                 & 128               & 1                \\
\hline
BiLSTM & 0.0001        & 8                  & 64                & 1                \\
\hline
GRU    & 0.0001        & 8                  & 32                & 1                \\ 
\bottomrule[1.5pt]
\end{tabular}
\label{tab:baseline_models}
\end{center}
\end{table}

% \begin{table}[H]
%     \begin{center}
%     \caption*{Supplementary table 1: Summary of genomic surveillance report }
%     \label{tab:hyperparams}
%     \setlength{\tabcolsep}{8pt} % Default value: 6pt (column spacing)
%     \renewcommand{\arraystretch}{1.5} % Default value: 1 (row spacing)
%     \resizebox{0.5\textwidth}{!}{
%     \begin{tabular}{c|c|c|c}
%     \toprule[1.5pt]
%     \textbf{Variant} & \textbf{Release date} & \textbf{Source} & \textbf{Reference} \\
%     \hline
%     BA.2 & Feb 22, 2022 & WHO & \cite{BA2}\\
%     \hline
%     BA.4 & May 13, 2022 & ECDC & \cite{BA4_5}\\
%     \hline
%     BA.5 & May 13, 2022 & ECDC & \cite{BA4_5}\\
%     \hline
%     XBB & Oct 27, 2022 & WHO & \cite{who_bq}\\
%     \hline
%     BQ.1 & Oct 27, 2022 & WHO & \cite{who_bq}\\

%     \bottomrule[1.5pt]
%     \end{tabular}
%     }
%     \end{center}
% \end{table}

==> tables/genomic_report.tex <==
\begin{table}[H]
\small
    \begin{center}
    \caption*{Supplementary table 1: Summary of genomic surveillance report }
    \label{tab:genomic_report}
    \setlength{\tabcolsep}{8pt} % Default value: 6pt (column spacing)
    \renewcommand{\arraystretch}{1.5} % Default value: 1 (row spacing)
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{c|c|c|c}
    \toprule[1.5pt]
    \textbf{Variant} & \textbf{Release date} & \textbf{Source} & \textbf{Reference} \\
    \hline
    BA.2 & Feb 22, 2022 & WHO & \cite{BA2}\\
    \hline
    BA.4 & May 13, 2022 & ECDC & \cite{BA4_5}\\
    \hline
    BA.5 & May 13, 2022 & ECDC & \cite{BA4_5}\\
    \hline
    XBB & Oct 27, 2022 & WHO & \cite{who_bq}\\
    \hline
    BQ.1 & Oct 27, 2022 & WHO & \cite{who_bq}\\

    \bottomrule[1.5pt]
    \end{tabular}
    }
    \end{center}
\end{table}


==> tables/hyperparams.tex <==
\begin{table}[H]
    \begin{center}
    \caption*{Supplementary Table 3: Hyperparameters settings for \models. }
    \label{tab:hyperparams}
    \setlength{\tabcolsep}{4pt} % Default value: 6pt (column spacing)
    \renewcommand{\arraystretch}{1.1} % Default value: 1 (row spacing)
    \resizebox{0.9\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    \toprule[1.5pt]
     \multirow{2}{*}{\makecell[c]{\textbf{Prediction Target}}} & \multirow{2}{*}{\textbf{Model}} & \multicolumn{4}{c}{\textbf{Hyperparameters}}\\
     \cline{3-6}
      & & \textbf{Learning Rate} & \textbf{Random Seed} & \textbf{Static Information Augmentation}  & \textbf{Dynamic Information Augmentation}
      \\
      
      \hline
      
\multirow{3}{*}{1-week}
&\model-7B & 2e-5 & 2024 &  &  \\
&\model-13B & 1e-5 & 2023 & \checkmark &  \\
&\model-70B & 1e-5 & 2023 & \checkmark & \checkmark \\
 \cline{1-6}
  
\multirow{3}{*}{3-week}
&\model-7B & 2e-5 & 2024 & \checkmark &  \\
&\model-13B & 2e-5 & 2023 &  &  \\
&\model-70B & 2e-5 & 2023 & \checkmark & \checkmark \\
    \bottomrule[1.5pt]
    \end{tabular}
    }
    \end{center}
\end{table}


==> tables/result.tex <==
% \newpage
% \begin{table}[H]

%     \begin{subtable}{\textwidth}
%     \begin{center}
%     \subcaption{The \model\ Framework Result Summarization and Comparison with SOTA Methods on Grid-based Datasets}
%     \small
%     \setlength{\tabcolsep}{4pt} % Default value: 6pt (column spacing)
%     \renewcommand{\arraystretch}{1.1} % Default value: 1 (row spacing)
%     \resizebox{0.66\textwidth}{!}{
%     \begin{tabular}{c|c|c|c|c|c}
%     \toprule[1.5pt]
%      \multirow{2}{*}{\makecell[c]{\textbf{Data Type}}} & \multirow{2}{*}{\textbf{Cities}} & \multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{Evaluation Matrix}}\\
%      \cline{4-6}
%       & & & \textbf{MAE} $\downarrow$ & \textbf{MAPE (\%)} $\downarrow$ & \textbf{RMSE} $\downarrow$ \\\hline
      
%     \multirow{28}{*}{\makecell[c]{\textbf{Grid-based Data}}}
    
%     & \multirow{7}{*}{\makecell[c]{\textbf{Berlin Downtown}\\ (1024 grid, 10.32 km²)}} & 
%       UNet2D and LSTM \cite{liu2017short}  & 0.241 & 16.2 & 0.356 \\
%      && UNet3D \cite{choi2019traffic}  & 0.235 & 15.8 & 0.347   \\
%      &&  Vision Transformer \cite{dosovitskiy2020image} &0.192 & 13.0 & 0.284  \\
%       &&  Video Transformer \cite{arnab2021vivit} & 0.189 & 12.8 & 0.280 \\
%       & &  Swin Transformer \cite{liu2021swin} & 0.198 & 13.4 & 0.293  \\
%     %   & & \cellcolor{green!10}\model\ (proposed) w/o Edge & \cellcolor{green!10}\textbf{0.188} & \cellcolor{green!10}\textbf{0.127} & \cellcolor{green!10}\textbf{0.277} \\
%       & & \cellcolor{green!10}\model\ (proposed) & \cellcolor{green!10}\textbf{0.182} & \cellcolor{green!10}\textbf{12.3} & \cellcolor{green!10}\textbf{0.269} \\ \cline{2-6} 
      
%     & \multirow{7}{*}{\makecell[c]{\textbf{Berlin Rural Area (TBD)}\\ (1024 grid, 10.32 km²)}} & 
%       UNet2D and LSTM \cite{liu2017short}  & 0.249 & 16.7 & 0.366 \\
%      && UNet3D \cite{choi2019traffic}  & 0.257 & 17.0 & 0.374   \\
%      &&  Vision Transformer \cite{dosovitskiy2020image} & 0.236 & 15.9 & 0.349  \\
%       &&  Video Transformer \cite{arnab2021vivit} & 0.243 & 16.4 & 0.359 \\
%       & &  Swin Transformer \cite{liu2021swin} & 0.238 & 16.0 & 0.352  \\
%     %   & & \cellcolor{green!10}\model\ (proposed) w/o Edge & \cellcolor{green!10}\textbf{0.227} & \cellcolor{green!10}\textbf{0.153} & \cellcolor{green!10}\textbf{0.336} \\
%        & & \cellcolor{green!10}\model\ (proposed) & \cellcolor{green!10}\textbf{0.222} & \cellcolor{green!10}\textbf{15.0} & \cellcolor{green!10}\textbf{0.328} \\\cline{2-6} 
      
%      & \multirow{7}{*}{\makecell[c]{\textbf{Istanbul Downtown}\\ (1024 grid, 10.32 km²)}} 
%      & UNet2D and LSTM  \cite{liu2017short} & 0.582 & 39.1 & 0.858 \\
%      && UNet3D \cite{choi2019traffic} & 0.652 & 43.8 & 0.959   \\
%      &&  Vision Transformer \cite{dosovitskiy2020image}& 0.536 & 36.2 & 0.794  \\
%       &&  Video Transformer \cite{arnab2021vivit}& 0.591 & 38.9 & 0.852  \\
%       & &  Swin Transformer \cite{liu2021swin}& 0.586 & 39.6 & 0.867  \\
%     %   & & \cellcolor{green!10} \model\ (proposed) w/o Edge & \cellcolor{green!10}\textbf{0.499} & \cellcolor{green!10}\textbf{0.337} & \cellcolor{green!10}\textbf{0.739} \\
%       & & \cellcolor{green!10}\model\ (proposed) & \cellcolor{green!10}\textbf{0.484} & \cellcolor{green!10}\textbf{32.7} & \cellcolor{green!10}\textbf{0.716} \\\cline{2-6} 
      
%      & \multirow{7}{*}{\makecell[c]{\textbf{Bangkok Downtown}\\ (1024 grid, 10.32 km²)}} & 
%       UNet2D and LSTM \cite{liu2017short} & 0.335 & 22.6 & 0.495 \\
%      && UNet3D  \cite{choi2019traffic} & 0.328 & 22.1 & 0.486   \\
%      &&  Vision Transformer \cite{dosovitskiy2020image}& 0.335 & 22.5 & 0.493  \\
%       &&  Video Transformer \cite{arnab2021vivit}& 0.335 & 22.5 & 0.494  \\
%       & &  Swin Transformer \cite{liu2021swin}& 0.321 & 21.7 & 0.475  \\
%     %   & & \cellcolor{green!10}\model\ (proposed) w/o Edge & \cellcolor{green!10}\textbf{0.313} & \cellcolor{green!10}\textbf{0.211} & \cellcolor{green!10}\textbf{0.464} \\
%       & & \cellcolor{green!10}\model\ (proposed) & \cellcolor{green!10}\textbf{0.308} & \cellcolor{green!10}\textbf{20.8} & \cellcolor{green!10}\textbf{0.456} \\
      
%     \bottomrule[1.5pt]
%         %   \rowcolor{green!10}\cellcolor{white} &  \rowcolor{green!10}\cellcolor{white}& \model\ (proposed) & \textbf{1.72} & \textbf{3.78} & \textbf{3.97} \\\cline{2-6} 

%     \end{tabular}
%     }
%     \end{center}
%     \end{subtable}
%     \\
%     \label{tab:performance:grid}
% \end{table}%

% \newpage

% \begin{table}
%     \label{tab:results all}
%     \vspace{0.5cm}
%     \begin{subtable}{\textwidth}
%     \caption{The \model\ Framework Result Summarization and Comparison with SOTA Methods on Graph-based Datasets}
%     \end{subtable}
%     \begin{subtable}{\textwidth}
%     \begin{center}
%     \subcaption{The \model\ Framework Result Summarization and Comparison with SOTA Methods on Graph-based Datasets}
%     \setlength{\tabcolsep}{4pt} % Default value: 6pt (column spacing)
%     \renewcommand{\arraystretch}{1.1} % Default value: 1 (row spacing)
%     \resizebox{0.73\textwidth}{!}{

%     \begin{tabular}{c|c|c|c|c|c}
%     \toprule[1.5pt]
%      \multirow{2}{*}{\makecell[c]{\textbf{Data Type}}} & \multirow{2}{*}{\textbf{Cities}} & \multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c}{\textbf{Evaluation Matrix}}\\
%      \cline{4-6}
%       & & & \textbf{MAE} $\downarrow$ & \textbf{MAPE (\%)} $\downarrow$ & \textbf{RMSE} $\downarrow$ \\\hline
%     \multirow{32}{*}{\makecell[c]{\textbf{Graph-based Data}}} &
    
%     \multirow{9}{*}{\makecell[c]{\textbf{San Francisco}\\ (1358 nodes, 13 freeways and highways)}} & 
%       LSTM \cite{ma2015long}& 3.45 & 7.14 & 6.03 \\
%      & & LSGC-LSTM \cite{cui2019traffic} & 3.65 & 6.89 & 6.11 \\
%      & &  SGC-LSTM \cite{chen2020tssrgcn} & 3.89 & 7.25 & 6.29 \\
%      & &  MSTGCN \cite{guo2019attention} & 2.39 & 5.31 & 4.80 \\
%      & &  ASTGCN \cite{guo2019attention} & 2.30 & 5.18 & 5.09 \\
%      & &  AGCRN \cite{bai2020adaptive} & 2.23 & 5.01 & 4.89 \\
%      & &  ASTGNN \cite{guo2021learning}& 1.92 & 4.21 & 4.21 \\
%      & & \cellcolor{green!10}\model\ (proposed) & \cellcolor{green!10}\textbf{1.69} & \cellcolor{green!10}\textbf{3.60} & \cellcolor{green!10}\textbf{3.70} \\\cline{2-6} 
      
%      &\multirow{9}{*}{\makecell[c]{\textbf{Los Angles Downtown}\\ (1432 nodes, 18 freeways and highways)}} & 
%       LSTM \cite{ma2015long}& 4.43 & 11.11 & 7.63  \\
%      & & LSGC-LSTM \cite{cui2019traffic} & 4.60 & 9.46 & 7.63 \\
%      & &  SGC-LSTM \cite{chen2020tssrgcn} & 4.73 & 9.60 & 7.73 \\
%      & &  MSTGCN \cite{guo2019attention} & 2.84 & 7.17 & 5.47 \\
%      & &  ASTGCN \cite{guo2019attention} & 2.81 & 6.87 & 5.80 \\
%      & &  AGCRN \cite{bai2020adaptive} & 2.63 & 6.64 & 5.53 \\
%      & &  ASTGNN \cite{guo2021learning}& 2.25 & 5.62 & 5.02 \\
%      & & \cellcolor{green!10} \model\ (proposed) & \cellcolor{green!10} \textbf{1.88} & \cellcolor{green!10} \textbf{3.96} & \cellcolor{green!10} \textbf{3.92} \\\cline{2-6} 
      
%      &\multirow{9}{*}{\makecell[c]{\textbf{California Rural Freeway}\\ (1432 nodes, 18 freeways and highways)}} & 
%       LSTM \cite{ma2015long}& 2.19 & 3.66 & 4.10  \\
%      & & LSGC-LSTM \cite{cui2019traffic} & 2.36 & 3.90 & 4.20 \\
%      & &  SGC-LSTM \cite{chen2020tssrgcn} & 2.25 & 3.72 & 4.14 \\
%      & &  MSTGCN \cite{guo2019attention} & 1.31 & 2.56 & 2.92 \\
%      & &  ASTGCN \cite{guo2019attention} & 1.32 & 2.67 & 3.15 \\
%      & &  AGCRN \cite{bai2020adaptive} & 1.25 & 2.43 & 2.91 \\
%      & &  ASTGNN \cite{guo2021learning}& 1.01 & 2.00 & 2.71 \\
%      & & \cellcolor{green!10} \model\ (proposed) & \cellcolor{green!10} \textbf{0.93} & \cellcolor{green!10} \textbf{1.74} & \cellcolor{green!10} \textbf{2.22} \\\cline{2-6} 
      
%      &\multirow{9}{*}{\makecell[c]{\textbf{San Diego}\\ (862 nodes, 9 freeways and highways)}} & 
%       LSTM \cite{ma2015long}& 2.61 & 4.91 & 4.96 \\
%      & &  LSGC-LSTM \cite{cui2019traffic}& 2.77 & 4.90 & 4.99 \\
%      & &  SGC-LSTM \cite{chen2020tssrgcn} & 2.81 & 4.99 & 5.07  \\
%      & &  MSTGCN \cite{guo2019attention} & 1.72 & 3.83 & 3.78 \\
%      & &  ASTGCN \cite{guo2019attention} & 1.68 & 4.03 & 3.91 \\
%      & &  AGCRN \cite{bai2020adaptive} & 1.54 & 3.31 & 3.69 \\
%      & &  ASTGNN \cite{guo2021learning} & 1.37 & 2.88 & 3.34  \\
%      & & \cellcolor{green!10} \model\ (proposed) & \cellcolor{green!10} \textbf{1.15} & \cellcolor{green!10} \textbf{2.32} & \cellcolor{green!10}\textbf{2.59} \\
    
%     \bottomrule[1.5pt]
%     \end{tabular}
%     }
%     \end{center}
%     \end{subtable}
    
%     \caption{The results on all datasets used in this paper. As can be seen in the table, the proposed method consistently achieved the best performance across both the graph data and the grid data. }
%     \label{tab:performance}
% \end{table}

==> tables/variant_result.tex <==
\begin{table}[H]
    \begin{center}
    \caption{3-Week Covid Prediction Results with Variant from 2022-10-24 to 2022-11-28. \Yang{I think all weeks' results look better.} $\uparrow$/$\downarrow$ denotes the larger/smaller metric denotes better performance.}
    \label{tab:performance:variant}
    \small
    \setlength{\tabcolsep}{4pt} % Default value: 6pt (column spacing)
    \renewcommand{\arraystretch}{1.1} % Default value: 1 (row spacing)
    \resizebox{0.75\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    \toprule[1.5pt]
 \multirow{2}{*}{\textbf{Model}} & \multicolumn{5}{c}{\textbf{Evaluation Matrix}}\\
     \cline{2-6}
      & \textbf{Accuracy $\uparrow$} & \textbf{MSE $\downarrow$} & \textbf{WMSE $\downarrow$}  & \textbf{Brier Score $\downarrow$} & \textbf{RPS$\downarrow$}\\\hline

% all weeks
% \model(7b) & 0.453 & 1.019 & 1.115 & 0.749 & 0.127 \\
% \model(7b)+variant & 0.468 & 0.786 & 0.955 & 0.690 & 0.111 \\
% \cline{1-6} 
% \model(13b) & 0.485 & 0.931 & 1.094 & 0.669 & 0.109 \\
% \model(13b)+variant & 0.464 & 0.760 & 0.908 & 0.695 & 0.106 \\

% 6 weeks
\model(7b) & 0.343 & 1.227 & 1.256 & 0.889 & 0.149 \\
\model(7b)+variant & 0.363 & 0.857 & 0.909 & 0.843 & 0.128 \\
\cline{1-6} 
\model(13b) & 0.383 & 1.207 & 1.272 & 0.770 & 0.129 \\
\model(13b)+variant & 0.393 & 0.737 & 0.844 & 0.763 & 0.113 \\
      
    \bottomrule[1.5pt]

    \end{tabular}
    }
    \end{center}
\end{table}


